Are Safety Guarantees in Neural Networks Safe? How to Compute Trustworthy Robustness Certifications

A primary challenge in AI safety is the existence of adversarial examples -- slightly distorted inputs that cause a neural network (NN) to misclassify. To mitigate this problem, recent research focuses on the computation of robustness certifications, which, for a given input, determine the largest distortion the input may receive without breaking the network's prediction. Robustness certifications can be interpreted as an axis-aligned hyper-rectangle (multi-dimensional intervals). Most existing approaches focus on maximizing the certification's volume, but recent intractability results prohibit the computation of volume-optimal certifications in reasonable time. We introduce the apothem measure and show how to compute apothem-optimal certifications in a linear number of calls to a NN verifier (oracle) w.r.t. the input domain's diameter. Moreover, we prove that we cannot have a volume-optimal, oracle-based algorithm, even if we discard the oracle costs. Also, we introduce dual certifications -- an interval including all instances of a class -- thus providing apothem-minimum upper bounds to a robustness certification. Further, we present the ParallelepipedoNN system, which we evaluate on the standard MNIST and Fashion MNIST benchmarks. A preliminary comparison with existing work on the same datasets reveals at least two-fold improvement w.r.t. the minimum edge length.

==> algorithms/cyclic-dichotomic.tex <==
\begin{algorithm}[t]
    % \toprule
    \DontPrintSemicolon
    \caption{$\mathbb{B}$--\textsc{TopDown Search}}
    \label{algo:cyclic-dichotomic}
    \KwInput{$\mathbf{x} \in \mathbb{F}$, the center of the uniform interval certification, and a percision constant $\delta > 0$.}
    \KwOutput{A maximally sound uniform interval certification}

    $\mathtt{low} \gets 0$; $\mathtt{high} \gets \mathcal{A}(\mathbb{F})$; 
    
    \While{$\mathtt{high} - \mathtt{low} > \delta$}{
        $\rho \gets (\mathtt{high} - \mathtt{low}) / 2$

        $B \gets \mathcal{B}(\mathbf{x}, \rho)$
        
        \uIf{$\exists \mathbf{x}^\prime$, s.t. $\mathbf{x}^\prime \models \mathscr{S}_{B, \mathcal{N}}$}{
            $\mathtt{high} \gets \rho$
        }
        \Else{
            $\mathtt{low} \gets \rho$
        }
    }
    
    \Return{$B$}
\end{algorithm}
